Deep Multi-Sensor Lane Detection

Reliable and accurate lane detection has been a long-standing problem in the field of autonomous driving. In recent years, many approaches have been developed that use images (or videos) as input and reason in image space. In this paper we argue that accurate image estimates do not translate to precise 3D lane boundaries, which are the input required by modern motion planning algorithms. To address this issue, we propose a novel deep neural network that takes advantage of both LiDAR and camera sensors and produces very accurate estimates directly in 3D space. We demonstrate the performance of our approach on both highways and in cities, and show very accurate estimates in complex scenarios such as heavy traffic (which produces occlusion), fork, merges and intersections.

==> gellert_writing.tex <==
% Writings of Gellert in a seperate file to prevent conflicts
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}

\Gellert{We have a rectified pinhole camera defined by its camera calibration matrix $K$ and its relative pose to the frame of the vehicle $R_v, t_v$. These parameters are fixed and are captured by the projection matrix of the camera $C=K [R_v | t_v]$. This projects each $\bP_v= (x_v, y_v, z_v, 1)^T$ point from the vehicle frame into homogeneous camera pixels as $\bp = C \bP $.
Since both the lidar points and the ground height estimation is defined in the vehicle frame, the only unknown needed for backprojecting the camera image onto the ground is the $z_v$ ground height.

The lidar image is $L$, where each pixel has 3 channels $L_{x,y}=(z_i, i, n)$, the min height points in a raster, the mean intensity and the number of points per raster. 
Then $\bz_v = F_z(L | \Theta_z)$ where $F_z$ is a deepnet parameterized by its $\Theta_z$ weights to predict the ground.

Then the backprojected camera image $I$ can be written as: 
$I_{bp} = \phi_W(I, F_z(L) | C)$, where $\phi_W$ is the warping doing the backprojection with bilinear interpolation as in spatial transformer networks \cite{SpatialTransformerNetwork}. 

Note that this operation is differentiable, thus the whole network can be trained end-to-end. 

Note that this assumes a 2D surface where occlusions are neglected. This can cause errors, e.g. backprojecting pixels of a car onto the ground, but since the class of interest, i.e. lanes, are by definition on the ground it will be accurate for those. 

We were experimenting with two settings, in the first we directly backproject the RGB image pixels to the ground and then input those into a net doing its predictions in the ortho-view space.
As second option, we calculate features in the original camera space and backproject the computed features and input them into the net defined in the ortho-view. 
Note that this needs end-to-end training which is feasible by our backprojecting method. 




\paragraph{Time aggregation:}

The aggregated output $A_t,i$ for each pixel i at time $t$ is calculated as mean of each observations for a given location.
To calculate this, the motion of the vehicle is considered end the output space is warped to the current frame by $\phi(E_t, z_t)$ depending on the $E_t = [R_t | t_t]$ rotation and translation to the previous frame. 
In the $\Psi$ transformation we transform each $P_{t,i}$ 3D point to previous frame by $E_t$ and ortho project it (omit the $z$ coordinate). This gives us a transformation for each point which can be used for warping the previous accumulated array $A_{t-1, i}$....

\begin{align}
A_t,i =  \frac{ n_i \phi_A(A_{t-1, i}, E_t) + y_{t, i}  )}{n_i+1}
\end{align}
where $n_i$ is counting how often a pixel $i$ was visible up to this time point. 

\paragraph{Figures to do}

\begin{enumerate}
\item Camera detection reprojected. 
\end{enumerate}





}
